A study on the combined interplay between stochastic fluctuations and the number of flagella in bacterial chemotaxis

The chemotactic pathway allows bacteria to respond and adapt to environmental changes, by tuning the tumbling and running motions that are due to clockwise and counterclockwise rotations of their flagella. The pathway is tightly regulated by feedback mechanisms governed by the phosphorylation and methylation of several proteins. In this paper, we present a detailed mechanistic model for chemotaxis, that considers all of its transmembrane and cytoplasmic components, and their mutual interactions. Stochastic simulations of the dynamics of a pivotal protein, CheYp, are performed by means of tau leaping algorithm. This approach is then used to investigate the interplay between the stochastic fluctuations of CheYp amount and the number of cellular flagella. Our results suggest that the combination of these factors might represent a relevant component for chemotaxis. Moreover, we study the pathway under various conditions, such as different methylation levels and ligand amounts, in order to test its adaptation response. Some issues for future work are finally discussed.

==> eptcsdata.tex <==
\providecommand{\event}{R.J.Back, I.Petre, E. de Vink (Eds.): Computational\\
Models for Cell Processes (CompMod 2009)}
\providecommand{\volume}{6}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{47}
\providecommand{\eid}{4}

